Computational prediction of lattice thermal conductivity -- a comparison of molecular dynamics and Boltzmann transport approaches

The predictive modeling of lattice thermal conductivity is of fundamental importance for the understanding and design of materials for a wide range of applications. Two major approaches, namely molecular dynamics (MD) simulations and calculations solving approximately the Boltzmann transport equation (BTE), have been developed to compute the lattice thermal conductivity. We present a detailed direct comparison of these two approaches, using as prototypical cases MgO and PbTe. The comparison, carried out using empirical potentials, takes into account the effects of fourth order phonon scattering, temperature-dependent phonon frequencies (phonon renormalization), and investigates the effects of quantum vs. classical statistics. We clarify that equipartition, as opposed to Maxwell Boltzmann, govern the statistics of phonons in MD simulations. We find that lattice thermal conductivity values from MD and BTE show an apparent, satisfactory agreement; however such an agreement is the result of error cancellations. We also show that the primary effect of statistics on thermal conductivity is via the scattering rate dependence on phonon populations.

==> bib.tex <==
% $ biblatex auxiliary file $
% $ biblatex bbl format version 2.5 $
% Do not modify the above lines!
%
% This is an auxiliary file used by the 'biblatex' package.
% This file may safely be deleted. It will be recreated by
% biber as required.
%
\begingroup
\makeatletter
\@ifundefined{ver@biblatex.sty}
  {\@latex@error
     {Missing 'biblatex' package}
     {The bibliography requires the 'biblatex' package.}
      \aftergroup\endinput}
  {}
\endgroup


\refsection{0}
  \sortlist{none}{none}
    \entry{Lu2016}{article}{}
      \name{author}{5}{}{%
        {{hash=c24892f508eb32848ee7f82202519e04}{Lu}{L\bibinitperiod}{Xiaodong}{X\bibinitperiod}{}{}{}{}}%
        {{hash=f0e7d180081df6c4c59c600f7c044474}{Zhao}{Z\bibinitperiod}{Yang}{Y\bibinitperiod}{}{}{}{}}%
        {{hash=8463a8cb4788379518946f4406584dbb}{Wang}{W\bibinitperiod}{Zelai}{Z\bibinitperiod}{}{}{}{}}%
        {{hash=3c4fc3151828c8c9afef926003acf26c}{Zhang}{Z\bibinitperiod}{Jinjing}{J\bibinitperiod}{}{}{}{}}%
        {{hash=7dacbb5a6e92ab16944d46ba03705563}{Song}{S\bibinitperiod}{Yang}{Y\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{85fd791f38e5bac99e822a8ce7159ed7}
      \strng{fullhash}{e96e4e7417b4057c6e6a325f8b17bc51}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{0038-092X}
      \field{journaltitle}{Solar Energy}
      \field{title}{Influence of environmental temperature and device temperature difference on output parameters of c-Si solar cells}
      \field{volume}{136}
      \field{year}{2016}
      \field{pages}{333\bibrangedash 341}
      \range{pages}{9}
      \keyw{Temperature}
    \endentry
    \entry{Modestino2015}{article}{}
      \name{author}{2}{}{%
        {{hash=d1a328c2892c652246da13466ced3a1f}{Modestino}{M\bibinitperiod}{Miguel\bibnamedelima A.}{M\bibinitperiod\bibinitdelim A\bibinitperiod}{}{}{}{}}%
        {{hash=a3c6d1534536c56e1d3c5e5fc4759fd9}{Haussener}{H\bibinitperiod}{Sophia}{S\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{2cf62518d27d590b54fbd87ee0bba890}
      \strng{fullhash}{2cf62518d27d590b54fbd87ee0bba890}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Annual Review of Chemical and Biomolecular Engineering}
      \field{note}{PMID: 26083057}
      \field{number}{1}
      \field{title}{An Integrated Device View on Photo-Electrochemical Solar-Hydrogen Generation}
      \field{volume}{6}
      \field{year}{2015}
      \field{pages}{13\bibrangedash 34}
      \range{pages}{22}
    \endentry
    \entry{Dresselhaus2007}{article}{}
      \name{author}{9}{}{%
        {{hash=0cbd423d1a733acdaf7624eccf35e408}{Dresselhaus}{D\bibinitperiod}{M.S.}{M\bibinitperiod}{}{}{}{}}%
        {{hash=269cebd970e6a5f308aa64d90fe877fe}{Chen}{C\bibinitperiod}{G.}{G\bibinitperiod}{}{}{}{}}%
        {{hash=0b86c1c5a3adc3678d14063be315e9ea}{Tang}{T\bibinitperiod}{M.Y.}{M\bibinitperiod}{}{}{}{}}%
        {{hash=21547f23b534546443fc3659d95a3462}{Yang}{Y\bibinitperiod}{R.G.}{R\bibinitperiod}{}{}{}{}}%
        {{hash=04db7d40a3548a4772e2af802c359b23}{Lee}{L\bibinitperiod}{H.}{H\bibinitperiod}{}{}{}{}}%
        {{hash=5c7e3b4dd846ffb7a934b964dbebdaa3}{Wang}{W\bibinitperiod}{D.Z.}{D\bibinitperiod}{}{}{}{}}%
        {{hash=e2c547dc70c8b1c4ecadc90d5562f1e2}{Ren}{R\bibinitperiod}{Z.F.}{Z\bibinitperiod}{}{}{}{}}%
        {{hash=0f2a598b99ecb8af165379a0128d581b}{Fleurial}{F\bibinitperiod}{J.-P.}{J\bibinithyphendelim P\bibinitperiod}{}{}{}{}}%
        {{hash=e2862e7d4290cc611e625da5ebe4a9bf}{Gogna}{G\bibinitperiod}{P.}{P\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {WILEY-VCH Verlag}%
      }
      \strng{namehash}{6b58f23159fd3fb3de450c95158535d7}
      \strng{fullhash}{8bb41d2cb012b228174b74f92224bfcd}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{1521-4095}
      \field{journaltitle}{Advanced Materials}
      \field{number}{8}
      \field{title}{New Directions for Low-Dimensional Thermoelectric Materials}
      \field{volume}{19}
      \field{year}{2007}
      \field{pages}{1043\bibrangedash 1053}
      \range{pages}{11}
      \keyw{Nanocomposites,Nanostructured materials,Quantum wells,Quantum-confinement effects,Thermoelectric materials}
    \endentry
    \entry{Fitriani2016}{article}{}
      \name{author}{8}{}{%
        {{hash=5437f2c2433aa86fd21b8381b0365ced}{Fitriani}{F\bibinitperiod}{}{}{}{}{}{}}%
        {{hash=cfb9c02ba99e9042852868607fbe3b69}{Ovik}{O\bibinitperiod}{R.}{R\bibinitperiod}{}{}{}{}}%
        {{hash=6510f8ecec46ac8c37a7ae96e4f2f288}{Long}{L\bibinitperiod}{B.D.}{B\bibinitperiod}{}{}{}{}}%
        {{hash=f899f68d10fbdb5942c19750726a68f3}{Barma}{B\bibinitperiod}{M.C.}{M\bibinitperiod}{}{}{}{}}%
        {{hash=8b8716840769ff990db1cf1dd4ede64d}{Riaz}{R\bibinitperiod}{M.}{M\bibinitperiod}{}{}{}{}}%
        {{hash=9747a93065a94ca8110a3c670efd1ed0}{Sabri}{S\bibinitperiod}{M.F.M.}{M\bibinitperiod}{}{}{}{}}%
        {{hash=de6ca0ee4a90916a87343bb054e1a3a6}{Said}{S\bibinitperiod}{S.M.}{S\bibinitperiod}{}{}{}{}}%
        {{hash=402e32fc0adb4bfbfc47a1aa929d448c}{Saidur}{S\bibinitperiod}{R.}{R\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{c110938cda784f19caf8af84d05b842c}
      \strng{fullhash}{dc17377aba47f01e191b42c5fd444681}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{1364-0321}
      \field{journaltitle}{Renewable and Sustainable Energy Reviews}
      \field{title}{A review on nanostructures of high-temperature thermoelectric materials for waste heat recovery}
      \field{volume}{64}
      \field{year}{2016}
      \field{pages}{635\bibrangedash 659}
      \range{pages}{25}
      \keyw{Waste heat recovery}
    \endentry
    \entry{Zebarjadi2016}{article}{}
      \name{author}{1}{}{%
        {{hash=497c8807def24366eb937c558a7327ba}{Zebarjadi}{Z\bibinitperiod}{M.}{M\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {Nature Publishing Group}%
      }
      \strng{namehash}{497c8807def24366eb937c558a7327ba}
      \strng{fullhash}{497c8807def24366eb937c558a7327ba}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{2045-2322}
      \field{journaltitle}{Sci Rep}
      \field{month}{04}
      \field{note}{27033717[pmid]}
      \field{title}{Heat Management in Thermoelectric Power Generators}
      \field{volume}{6}
      \field{year}{2016}
      \field{pages}{20951}
      \range{pages}{1}
    \endentry
    \entry{Minnich2011}{article}{}
      \name{author}{7}{}{%
        {{hash=6c32cb3affa9c4d8e0073b8fb981e58f}{Minnich}{M\bibinitperiod}{A.\bibnamedelimi J.}{A\bibinitperiod\bibinitdelim J\bibinitperiod}{}{}{}{}}%
        {{hash=e111deeecef4e134791e475322c3c115}{Johnson}{J\bibinitperiod}{J.\bibnamedelimi A.}{J\bibinitperiod\bibinitdelim A\bibinitperiod}{}{}{}{}}%
        {{hash=b0eccc00d81a190e412b8a5a328c8ea2}{Schmidt}{S\bibinitperiod}{A.\bibnamedelimi J.}{A\bibinitperiod\bibinitdelim J\bibinitperiod}{}{}{}{}}%
        {{hash=7b8f40799ddd1400985bc34b2788838a}{Esfarjani}{E\bibinitperiod}{K.}{K\bibinitperiod}{}{}{}{}}%
        {{hash=3e5430a7ad3e2d0b767d2feb2a717833}{Dresselhaus}{D\bibinitperiod}{M.\bibnamedelimi S.}{M\bibinitperiod\bibinitdelim S\bibinitperiod}{}{}{}{}}%
        {{hash=2726f8a67d9b860c74073f89d32b810e}{Nelson}{N\bibinitperiod}{K.\bibnamedelimi A.}{K\bibinitperiod\bibinitdelim A\bibinitperiod}{}{}{}{}}%
        {{hash=269cebd970e6a5f308aa64d90fe877fe}{Chen}{C\bibinitperiod}{G.}{G\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{6b4d2ad2bf651d6dd3dba3eb7a24230a}
      \strng{fullhash}{5fbf68169a192e5d3fbc0ac0a741548d}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{9}
      \field{journaltitle}{Phys. Rev. Lett.}
      \field{month}{08}
      \field{title}{Thermal Conductivity Spectroscopy Technique to Measure Phonon Mean Free Paths}
      \field{volume}{107}
      \field{year}{2011}
      \field{pages}{095901}
      \range{pages}{1}
    \endentry
    \entry{Zeng2015}{article}{}
      \name{author}{11}{}{%
        {{hash=201a80740b7e1afd052d0ce00eab7cb4}{Zeng}{Z\bibinitperiod}{Lingping}{L\bibinitperiod}{}{}{}{}}%
        {{hash=89a25273ec76eaf5fde4066ad91f2445}{Collins}{C\bibinitperiod}{Kimberlee\bibnamedelima C.}{K\bibinitperiod\bibinitdelim C\bibinitperiod}{}{}{}{}}%
        {{hash=c07e6fe655ddf2762a0264aa46c84958}{Hu}{H\bibinitperiod}{Yongjie}{Y\bibinitperiod}{}{}{}{}}%
        {{hash=7f857551cd418df59a285f223f8dc031}{Luckyanova}{L\bibinitperiod}{Maria\bibnamedelima N.}{M\bibinitperiod\bibinitdelim N\bibinitperiod}{}{}{}{}}%
        {{hash=b421d51c413d17e96dbe29a259eafdde}{Maznev}{M\bibinitperiod}{Alexei\bibnamedelima A.}{A\bibinitperiod\bibinitdelim A\bibinitperiod}{}{}{}{}}%
        {{hash=3460bee6d554b1ad13006d710f512abd}{Huberman}{H\bibinitperiod}{Samuel}{S\bibinitperiod}{}{}{}{}}%
        {{hash=a433499e96e1631b76eb4b1a7bb5cd1b}{Chiloyan}{C\bibinitperiod}{Vazrik}{V\bibinitperiod}{}{}{}{}}%
        {{hash=4ef041d359c37f80515dd829d331aadb}{Zhou}{Z\bibinitperiod}{Jiawei}{J\bibinitperiod}{}{}{}{}}%
        {{hash=1143efecc9d5b33cc2cc9122ceca7045}{Huang}{H\bibinitperiod}{Xiaopeng}{X\bibinitperiod}{}{}{}{}}%
        {{hash=49777a289be75aa24a5fdc5647761bde}{Nelson}{N\bibinitperiod}{Keith\bibnamedelima A.}{K\bibinitperiod\bibinitdelim A\bibinitperiod}{}{}{}{}}%
        {{hash=293c31f46eb012efc4b2449215c92484}{Chen}{C\bibinitperiod}{Gang}{G\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {The Author(s) SN -}%
      }
      \strng{namehash}{8ef9a4b280303d20681389bdb3061b7e}
      \strng{fullhash}{cc630ff2ac4b70f5bca419eeabc296b8}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Scientific Reports}
      \field{month}{11}
      \field{note}{Article}
      \field{title}{Measuring Phonon Mean Free Path Distributions by Probing Quasiballistic Phonon Transport in Grating Nanostructures}
      \field{volume}{5}
      \field{year}{2015}
      \field{pages}{17131}
      \range{pages}{1}
    \endentry
    \entry{Chiloyan2016}{article}{}
      \name{author}{6}{}{%
        {{hash=a433499e96e1631b76eb4b1a7bb5cd1b}{Chiloyan}{C\bibinitperiod}{Vazrik}{V\bibinitperiod}{}{}{}{}}%
        {{hash=201a80740b7e1afd052d0ce00eab7cb4}{Zeng}{Z\bibinitperiod}{Lingping}{L\bibinitperiod}{}{}{}{}}%
        {{hash=3460bee6d554b1ad13006d710f512abd}{Huberman}{H\bibinitperiod}{Samuel}{S\bibinitperiod}{}{}{}{}}%
        {{hash=b421d51c413d17e96dbe29a259eafdde}{Maznev}{M\bibinitperiod}{Alexei\bibnamedelima A.}{A\bibinitperiod\bibinitdelim A\bibinitperiod}{}{}{}{}}%
        {{hash=49777a289be75aa24a5fdc5647761bde}{Nelson}{N\bibinitperiod}{Keith\bibnamedelima A.}{K\bibinitperiod\bibinitdelim A\bibinitperiod}{}{}{}{}}%
        {{hash=293c31f46eb012efc4b2449215c92484}{Chen}{C\bibinitperiod}{Gang}{G\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{a2af3fd675a3d6c6ecacb3d3c9af8daf}
      \strng{fullhash}{9c84705af80ceb58d0135f457b415d51}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{15}
      \field{journaltitle}{Phys. Rev. B}
      \field{month}{04}
      \field{title}{Variational approach to extracting the phonon mean free path distribution from the spectral Boltzmann transport equation}
      \field{volume}{93}
      \field{year}{2016}
      \field{pages}{155201}
      \range{pages}{1}
    \endentry
    \entry{Broido2007}{article}{}
      \name{author}{5}{}{%
        {{hash=700402ff006b20154352657a2e5b0ea8}{Broido}{B\bibinitperiod}{D.\bibnamedelimi A.}{D\bibinitperiod\bibinitdelim A\bibinitperiod}{}{}{}{}}%
        {{hash=b2dc01da4234a026a60541bc4c35d736}{Malorny}{M\bibinitperiod}{M.}{M\bibinitperiod}{}{}{}{}}%
        {{hash=61814d121123d3aa5c0c8572bd13984b}{Birner}{B\bibinitperiod}{G.}{G\bibinitperiod}{}{}{}{}}%
        {{hash=e600b3ad4e78d119cbf3351a5c2d79fb}{Mingo}{M\bibinitperiod}{Natalio}{N\bibinitperiod}{}{}{}{}}%
        {{hash=3be043eeccec941b23ab94cf6f631a2e}{Stewart}{S\bibinitperiod}{D.\bibnamedelimi A.}{D\bibinitperiod\bibinitdelim A\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{9f59dc18df698caad8f6630477d1ee06}
      \strng{fullhash}{13debb271e0f12750aa207a928220d2d}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{eid}{231922}
      \field{journaltitle}{Applied Physics Letters}
      \field{number}{23}
      \field{title}{Intrinsic lattice thermal conductivity of semiconductors from first principles}
      \field{volume}{91}
      \field{year}{2007}
    \endentry
    \entry{Garg2011}{article}{}
      \name{author}{4}{}{%
        {{hash=788486622bdfcb165cb87cbb92c2ba0d}{Garg}{G\bibinitperiod}{Jivtesh}{J\bibinitperiod}{}{}{}{}}%
        {{hash=7d66e07674d0f438cfca3242e5b1d7f0}{Bonini}{B\bibinitperiod}{Nicola}{N\bibinitperiod}{}{}{}{}}%
        {{hash=0b6025fed4b33cd56ba34b371d229b3f}{Kozinsky}{K\bibinitperiod}{Boris}{B\bibinitperiod}{}{}{}{}}%
        {{hash=789148b9644893e2b07e550eec09d89c}{Marzari}{M\bibinitperiod}{Nicola}{N\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{2350da9df34367ea3f616761821fdd2a}
      \strng{fullhash}{83adb20898fe8afedf5e4dedb55e3d18}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{4}
      \field{journaltitle}{Phys. Rev. Lett.}
      \field{month}{01}
      \field{title}{Role of Disorder and Anharmonicity in the Thermal Conductivity of Silicon-Germanium Alloys: A First-Principles Study}
      \field{volume}{106}
      \field{year}{2011}
      \field{pages}{045901}
      \range{pages}{1}
    \endentry
    \entry{Marcolongo2016}{article}{}
      \name{author}{3}{}{%
        {{hash=504ff749edfd8eee91cedc6dd5c8a916}{Marcolongo}{M\bibinitperiod}{Aris}{A\bibinitperiod}{}{}{}{}}%
        {{hash=39e30f81debbdc72b93a09eabebc2808}{Umari}{U\bibinitperiod}{Paolo}{P\bibinitperiod}{}{}{}{}}%
        {{hash=c6d9ba190821969a9596dbde06ea38db}{Baroni}{B\bibinitperiod}{Stefano}{S\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{30aed8c6e51abb0b012d16c555588d63}
      \strng{fullhash}{30aed8c6e51abb0b012d16c555588d63}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{1745-2473}
      \field{journaltitle}{Nature Physics}
      \field{number}{1}
      \field{title}{Microscopic theory and quantum simulation of atomic heat transport}
      \field{volume}{12}
      \field{year}{2016}
      \field{pages}{80\bibrangedash 84}
      \range{pages}{5}
    \endentry
    \entry{Carbogno2016}{article}{}
      \name{author}{3}{}{%
        {{hash=ba966d0f7cb3da92d543134ea0684a5d}{Carbogno}{C\bibinitperiod}{Christian}{C\bibinitperiod}{}{}{}{}}%
        {{hash=f29400917315d357d6ac48f9df3520b0}{Ramprasad}{R\bibinitperiod}{Rampi}{R\bibinitperiod}{}{}{}{}}%
        {{hash=b39fc67a3375766bfd10f3b489a3d909}{Scheffler}{S\bibinitperiod}{Matthias}{M\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{848f4d0f6aa260a68ca5246788344f48}
      \strng{fullhash}{848f4d0f6aa260a68ca5246788344f48}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{17}
      \field{journaltitle}{Phys. Rev. Lett.}
      \field{month}{04}
      \field{title}{Ab Initio}
      \field{volume}{118}
      \field{year}{2017}
      \field{pages}{175901}
      \range{pages}{1}
    \endentry
    \entry{Cepellotti2016}{article}{}
      \name{author}{2}{}{%
        {{hash=333bf1bc88422fbb55eb505912b8159a}{Cepellotti}{C\bibinitperiod}{Andrea}{A\bibinitperiod}{}{}{}{}}%
        {{hash=789148b9644893e2b07e550eec09d89c}{Marzari}{M\bibinitperiod}{Nicola}{N\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{7c21e75457c2fa570843c9f2668913e8}
      \strng{fullhash}{7c21e75457c2fa570843c9f2668913e8}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{4}
      \field{journaltitle}{Phys. Rev. X}
      \field{month}{10}
      \field{title}{Thermal Transport in Crystals as a Kinetic Theory of Relaxons}
      \field{volume}{6}
      \field{year}{2016}
      \field{pages}{041013}
      \range{pages}{1}
    \endentry
    \entry{Zhou2014}{article}{}
      \name{author}{4}{}{%
        {{hash=7c8ea78b26e5365d21c23659d9b4f074}{Zhou}{Z\bibinitperiod}{Fei}{F\bibinitperiod}{}{}{}{}}%
        {{hash=a0934e662b9fab3c4dbd7dab102ffc42}{Nielson}{N\bibinitperiod}{Weston}{W\bibinitperiod}{}{}{}{}}%
        {{hash=9872d4238a18e9b8e34274bb6da5f0e4}{Xia}{X\bibinitperiod}{Yi}{Y\bibinitperiod}{}{}{}{}}%
        {{hash=3b8b82e57267e07be69c2d6651622567}{Ozoli\ifmmode\bibnamedelimb \mbox{ņ}\else\bibnamedelimb ņ\fi{}\ifmmode\bibnamedelimb \check{s}\else\bibnamedelima š\fi{}}{O\bibinitperiod\bibinitdelim \~ņ\bibinitperiod\bibinitdelim \~š\bibinitperiod}{Vidvuds}{V\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{da0c57ee4764d3eb901c39db7eec9eaf}
      \strng{fullhash}{a658f27f29d0c8f3af3c310ed946b1f6}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{18}
      \field{journaltitle}{Phys. Rev. Lett.}
      \field{month}{10}
      \field{title}{Lattice Anharmonicity and Thermal Conductivity from Compressive Sensing of First-Principles Calculations}
      \field{volume}{113}
      \field{year}{2014}
      \field{pages}{185501}
      \range{pages}{1}
    \endentry
    \entry{Stackhouse2010}{article}{}
      \name{author}{3}{}{%
        {{hash=0bc2dfc8c71685dccae8ee22672fc954}{Stackhouse}{S\bibinitperiod}{Stephen}{S\bibinitperiod}{}{}{}{}}%
        {{hash=21d34dbb1f274b088f6019d750c42e8c}{Stixrude}{S\bibinitperiod}{Lars}{L\bibinitperiod}{}{}{}{}}%
        {{hash=ff8608457d70bd404a7cb08f92946dd2}{Karki}{K\bibinitperiod}{Bijaya\bibnamedelima B.}{B\bibinitperiod\bibinitdelim B\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{6b897ab8df82c3e14cd413d319c3f721}
      \strng{fullhash}{6b897ab8df82c3e14cd413d319c3f721}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{20}
      \field{journaltitle}{Phys. Rev. Lett.}
      \field{month}{05}
      \field{title}{Thermal Conductivity of Periclase (MgO) from First Principles}
      \field{volume}{104}
      \field{year}{2010}
      \field{pages}{208501}
      \range{pages}{1}
    \endentry
    \entry{Cahill2014}{article}{}
      \name{author}{14}{}{%
        {{hash=561b1529fad7d4f0a364b8f8ba7e57b6}{Cahill}{C\bibinitperiod}{David\bibnamedelima G.}{D\bibinitperiod\bibinitdelim G\bibinitperiod}{}{}{}{}}%
        {{hash=cdda0372b2bf31ddbd3ab66cba2c0fa4}{Braun}{B\bibinitperiod}{Paul\bibnamedelima V.}{P\bibinitperiod\bibinitdelim V\bibinitperiod}{}{}{}{}}%
        {{hash=293c31f46eb012efc4b2449215c92484}{Chen}{C\bibinitperiod}{Gang}{G\bibinitperiod}{}{}{}{}}%
        {{hash=1c1fa2267e885aa9b5e15f10300e2450}{Clarke}{C\bibinitperiod}{David\bibnamedelima R.}{D\bibinitperiod\bibinitdelim R\bibinitperiod}{}{}{}{}}%
        {{hash=f949287454ec425b0cf7493a1d881de9}{Fan}{F\bibinitperiod}{Shanhui}{S\bibinitperiod}{}{}{}{}}%
        {{hash=9e5cbc50aacbe6534d89a709782bf277}{Goodson}{G\bibinitperiod}{Kenneth\bibnamedelima E.}{K\bibinitperiod\bibinitdelim E\bibinitperiod}{}{}{}{}}%
        {{hash=ebf62a6c95a9ef8821da65b778125980}{Keblinski}{K\bibinitperiod}{Pawel}{P\bibinitperiod}{}{}{}{}}%
        {{hash=6e3424612f782d37f87ad289cecfe21b}{King}{K\bibinitperiod}{William\bibnamedelima P.}{W\bibinitperiod\bibinitdelim P\bibinitperiod}{}{}{}{}}%
        {{hash=c1d5d4e41688cfe898f810b1ed4d4270}{Mahan}{M\bibinitperiod}{Gerald\bibnamedelima D.}{G\bibinitperiod\bibinitdelim D\bibinitperiod}{}{}{}{}}%
        {{hash=0d0cf2969b1e91c77a82d0fb90651dca}{Majumdar}{M\bibinitperiod}{Arun}{A\bibinitperiod}{}{}{}{}}%
        {{hash=76b1672c64a4d0d900a8a966f0a1fe9a}{Maris}{M\bibinitperiod}{Humphrey\bibnamedelima J.}{H\bibinitperiod\bibinitdelim J\bibinitperiod}{}{}{}{}}%
        {{hash=d56395fa0c9d5882660fe99727b4de86}{Phillpot}{P\bibinitperiod}{Simon\bibnamedelima R.}{S\bibinitperiod\bibinitdelim R\bibinitperiod}{}{}{}{}}%
        {{hash=288efd65c91c298f33226d5b96dd3c2e}{Pop}{P\bibinitperiod}{Eric}{E\bibinitperiod}{}{}{}{}}%
        {{hash=cfd4887b4262b2b11bafee4fd013ab4b}{Shi}{S\bibinitperiod}{Li}{L\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{f0eb47f6cb902b4f4adcd0d0fe32f177}
      \strng{fullhash}{0e55328090cd0f1975cf90e6dad50882}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{eid}{011305}
      \field{journaltitle}{Applied Physics Reviews}
      \field{number}{1}
      \field{title}{Nanoscale thermal transport. II. 2003–2012}
      \field{volume}{1}
      \field{year}{2014}
    \endentry
    \entry{Cahill1990}{article}{}
      \name{author}{1}{}{%
        {{hash=561b1529fad7d4f0a364b8f8ba7e57b6}{Cahill}{C\bibinitperiod}{David\bibnamedelima G.}{D\bibinitperiod\bibinitdelim G\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{561b1529fad7d4f0a364b8f8ba7e57b6}
      \strng{fullhash}{561b1529fad7d4f0a364b8f8ba7e57b6}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Review of Scientific Instruments}
      \field{number}{2}
      \field{title}{Thermal conductivity measurement from 30 to 750 K: the 3$\omega$ method}
      \field{volume}{61}
      \field{year}{1990}
      \field{pages}{802\bibrangedash 808}
      \range{pages}{7}
    \endentry
    \entry{Jiang2016}{article}{}
      \name{author}{3}{}{%
        {{hash=fb1282e2e9b631acba908570c8986a93}{Jiang}{J\bibinitperiod}{Puqing}{P\bibinitperiod}{}{}{}{}}%
        {{hash=77a6a3939d12fd1d95b8a8dcf1d8dd3a}{Lindsay}{L\bibinitperiod}{Lucas}{L\bibinitperiod}{}{}{}{}}%
        {{hash=77e37bbed3bb8b464e1343bfdb5ba315}{Koh}{K\bibinitperiod}{Yee\bibnamedelima Kan}{Y\bibinitperiod\bibinitdelim K\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{226a5eace5f6832b94fe66337970d046}
      \strng{fullhash}{226a5eace5f6832b94fe66337970d046}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{eid}{245705}
      \field{journaltitle}{Journal of Applied Physics}
      \field{number}{24}
      \field{title}{Role of low-energy phonons with mean-free-paths $ > \;0.8 \mu$m in heat conduction in silicon}
      \field{volume}{119}
      \field{year}{2016}
    \endentry
    \entry{Omini1995}{article}{}
      \name{author}{2}{}{%
        {{hash=47b5c119a88f17d20bec21c287bbe4b0}{Omini}{O\bibinitperiod}{M}{M\bibinitperiod}{}{}{}{}}%
        {{hash=91284d58c3a3e61736a4e45c61230d37}{Sparavigna}{S\bibinitperiod}{A}{A\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{036730b02bd7e5869797c687e9a288c4}
      \strng{fullhash}{036730b02bd7e5869797c687e9a288c4}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{0921-4526}
      \field{journaltitle}{Physica B: Condensed Matter}
      \field{number}{2}
      \field{title}{An iterative approach to the phonon Boltzmann equation in the theory of thermal conductivity}
      \field{volume}{212}
      \field{year}{1995}
      \field{pages}{101\bibrangedash 112}
      \range{pages}{12}
    \endentry
    \entry{Fugallo2013}{article}{}
      \name{author}{4}{}{%
        {{hash=bb2bf5bffb824ba074ad618fd5da7123}{Fugallo}{F\bibinitperiod}{Giorgia}{G\bibinitperiod}{}{}{}{}}%
        {{hash=8c2690776de302e4098d7405bf6393de}{Lazzeri}{L\bibinitperiod}{Michele}{M\bibinitperiod}{}{}{}{}}%
        {{hash=aedc8b2082f0772ce2d152c70c04d545}{Paulatto}{P\bibinitperiod}{Lorenzo}{L\bibinitperiod}{}{}{}{}}%
        {{hash=10f05ef61dea941f44620ab6ca249da6}{Mauri}{M\bibinitperiod}{Francesco}{F\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{95168cc3aed91f0078732e6d73732780}
      \strng{fullhash}{1e919dc705a41efaa8f0cd66fc3ab1b4}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{4}
      \field{journaltitle}{Phys. Rev. B}
      \field{month}{07}
      \field{title}{\textit{Ab initio} variational approach for evaluating lattice thermal conductivity}
      \field{volume}{88}
      \field{year}{2013}
      \field{pages}{045430}
      \range{pages}{1}
    \endentry
    \entry{Callaway1959}{article}{}
      \name{author}{1}{}{%
        {{hash=728fb30969eab49b82855c94db0d6958}{Callaway}{C\bibinitperiod}{Joseph}{J\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{728fb30969eab49b82855c94db0d6958}
      \strng{fullhash}{728fb30969eab49b82855c94db0d6958}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{4}
      \field{journaltitle}{Phys. Rev.}
      \field{month}{02}
      \field{title}{Model for Lattice Thermal Conductivity at Low Temperatures}
      \field{volume}{113}
      \field{year}{1959}
      \field{pages}{1046\bibrangedash 1051}
      \range{pages}{6}
    \endentry
    \entry{MarcolongoThesis2014}{thesis}{}
      \name{author}{3}{}{%
        {{hash=504ff749edfd8eee91cedc6dd5c8a916}{Marcolongo}{M\bibinitperiod}{Aris}{A\bibinitperiod}{}{}{}{}}%
        {{hash=c6d9ba190821969a9596dbde06ea38db}{Baroni}{B\bibinitperiod}{Stefano}{S\bibinitperiod}{}{}{}{}}%
        {{hash=39e30f81debbdc72b93a09eabebc2808}{Umari}{U\bibinitperiod}{Paolo}{P\bibinitperiod}{}{}{}{}}%
      }
      \list{institution}{1}{%
        {International School for Advanced Study, via Bonomea 265, 34136 Trieste - Italy}%
      }
      \strng{namehash}{401fa5ba98ad1b2a36bf39fa07e7106c}
      \strng{fullhash}{401fa5ba98ad1b2a36bf39fa07e7106c}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{title}{Theory and Ab Inito simulation of Atomic Heat Transport}
      \field{type}{phdthesis}
      \field{year}{2014}
    \endentry
    \entry{Muller1997}{article}{}
      \name{author}{1}{}{%
        {{hash=4adaf82741a34934a97c2c6ebd40a98d}{Müller-Plathe}{M\bibinithyphendelim P\bibinitperiod}{Florian}{F\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{4adaf82741a34934a97c2c6ebd40a98d}
      \strng{fullhash}{4adaf82741a34934a97c2c6ebd40a98d}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{The Journal of Chemical Physics}
      \field{number}{14}
      \field{title}{A simple nonequilibrium molecular dynamics method for calculating the thermal conductivity}
      \field{volume}{106}
      \field{year}{1997}
      \field{pages}{6082\bibrangedash 6085}
      \range{pages}{4}
    \endentry
    \entry{Lampin2013}{article}{}
      \name{author}{4}{}{%
        {{hash=1f175ba013111b171a83b1051e195d16}{Lampin}{L\bibinitperiod}{E.}{E\bibinitperiod}{}{}{}{}}%
        {{hash=215ae8797a095c7970be99953a2725ae}{Palla}{P\bibinitperiod}{P.\bibnamedelimi L.}{P\bibinitperiod\bibinitdelim L\bibinitperiod}{}{}{}{}}%
        {{hash=23af809ae2b6bc2443a614413d827e52}{Francioso}{F\bibinitperiod}{P.-A.}{P\bibinithyphendelim A\bibinitperiod}{}{}{}{}}%
        {{hash=6036b0d72dc3f5e0a56bf13b37c03487}{Cleri}{C\bibinitperiod}{F.}{F\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{fb6c7c119859b0b6bb6cb8980a65572e}
      \strng{fullhash}{c37c215fe35ecda34cd123749299b5e4}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{eid}{033525}
      \field{journaltitle}{Journal of Applied Physics}
      \field{number}{3}
      \field{title}{Thermal conductivity from approach-to-equilibrium molecular dynamics}
      \field{volume}{114}
      \field{year}{2013}
    \endentry
    \entry{Melis2014}{article}{}
      \name{author}{4}{}{%
        {{hash=8c1c75a2d38ce4d8fabd194ecc57a571}{{Melis,\bibnamedelimb Claudio}}{M\bibinitperiod}{}{}{}{}{}{}}%
        {{hash=37d97bf17e0f86ef45639ea6d3ea03a4}{{Dettori,\bibnamedelimb Riccardo}}{D\bibinitperiod}{}{}{}{}{}{}}%
        {{hash=ff67f25db6e7ef5ec199559f0052b4b3}{{Vandermeulen,\bibnamedelimb Simon}}{V\bibinitperiod}{}{}{}{}{}{}}%
        {{hash=8226b13f6e8d7b52ea92b56f084b1691}{{Colombo,\bibnamedelimb Luciano}}{C\bibinitperiod}{}{}{}{}{}{}}%
      }
      \strng{namehash}{d1f340abd28dd6e1329b46c043094ff4}
      \strng{fullhash}{649e25e9d1f62124ee64efc167ad2a90}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Eur. Phys. J. B}
      \field{number}{4}
      \field{title}{Calculating thermal conductivity in a transient conduction regime: theory and implementation}
      \field{volume}{87}
      \field{year}{2014}
      \field{pages}{96}
      \range{pages}{1}
      \verb{doi}
      \verb 10.1140/epjb/e2014-50119-0
      \endverb
    \endentry
    \entry{Melis2014b}{article}{}
      \name{author}{2}{}{%
        {{hash=f6346d955920ec5a1960d1642c16cc3d}{Melis}{M\bibinitperiod}{Claudio}{C\bibinitperiod}{}{}{}{}}%
        {{hash=1f1577d1c435291738552646eb1411c1}{Colombo}{C\bibinitperiod}{Luciano}{L\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{7c90989cd907e13d8ff2911af2f223d1}
      \strng{fullhash}{7c90989cd907e13d8ff2911af2f223d1}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{6}
      \field{journaltitle}{Phys. Rev. Lett.}
      \field{month}{02}
      \field{title}{Lattice Thermal Conductivity of ${\mathrm{Si}}_{1\ensuremath{-}x}{\mathrm{Ge}}_{x}$ Nanocomposites}
      \field{volume}{112}
      \field{year}{2014}
      \field{pages}{065901}
      \range{pages}{1}
    \endentry
    \entry{Barbarino2014}{article}{}
      \name{author}{3}{}{%
        {{hash=fdfebe7144eee30b7bc34d19718d9c09}{Barbarino}{B\bibinitperiod}{Giuliana}{G\bibinitperiod}{}{}{}{}}%
        {{hash=f6346d955920ec5a1960d1642c16cc3d}{Melis}{M\bibinitperiod}{Claudio}{C\bibinitperiod}{}{}{}{}}%
        {{hash=1f1577d1c435291738552646eb1411c1}{Colombo}{C\bibinitperiod}{Luciano}{L\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{16de1afeb1e21a077a1723223aab2160}
      \strng{fullhash}{16de1afeb1e21a077a1723223aab2160}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{0008-6223}
      \field{journaltitle}{Carbon}
      \field{title}{Effect of hydrogenation on graphene thermal transport}
      \field{volume}{80}
      \field{year}{2014}
      \field{pages}{167\bibrangedash 173}
      \range{pages}{7}
    \endentry
    \entry{Hahn2016}{article}{}
      \name{author}{3}{}{%
        {{hash=38f1529faea2b3df24befdd9876e365c}{Hahn}{H\bibinitperiod}{Konstanze\bibnamedelima R.}{K\bibinitperiod\bibinitdelim R\bibinitperiod}{}{}{}{}}%
        {{hash=f6346d955920ec5a1960d1642c16cc3d}{Melis}{M\bibinitperiod}{Claudio}{C\bibinitperiod}{}{}{}{}}%
        {{hash=1f1577d1c435291738552646eb1411c1}{Colombo}{C\bibinitperiod}{Luciano}{L\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{1ec91cda7104398988ea45b66c237ab1}
      \strng{fullhash}{1ec91cda7104398988ea45b66c237ab1}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{0008-6223}
      \field{journaltitle}{Carbon}
      \field{title}{Thermal transport in nanocrystalline graphene investigated by approach-to-equilibrium molecular dynamics simulations}
      \field{volume}{96}
      \field{year}{2016}
      \field{pages}{429\bibrangedash 438}
      \range{pages}{10}
    \endentry
    \entry{Barbarino2015}{article}{}
      \name{author}{3}{}{%
        {{hash=fdfebe7144eee30b7bc34d19718d9c09}{Barbarino}{B\bibinitperiod}{Giuliana}{G\bibinitperiod}{}{}{}{}}%
        {{hash=f6346d955920ec5a1960d1642c16cc3d}{Melis}{M\bibinitperiod}{Claudio}{C\bibinitperiod}{}{}{}{}}%
        {{hash=1f1577d1c435291738552646eb1411c1}{Colombo}{C\bibinitperiod}{Luciano}{L\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{16de1afeb1e21a077a1723223aab2160}
      \strng{fullhash}{16de1afeb1e21a077a1723223aab2160}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{3}
      \field{journaltitle}{Phys. Rev. B}
      \field{month}{01}
      \field{title}{Intrinsic thermal conductivity in monolayer graphene is ultimately upper limited: A direct estimation by atomistic simulations}
      \field{volume}{91}
      \field{year}{2015}
      \field{pages}{035416}
      \range{pages}{1}
    \endentry
    \entry{Xavier2016}{article}{}
      \name{author}{5}{}{%
        {{hash=be1716a6f19d52817258d858d30045f4}{Cartoixà}{C\bibinitperiod}{Xavier}{X\bibinitperiod}{}{}{}{}}%
        {{hash=05490348caeda328a6601f601c9330af}{Dettori}{D\bibinitperiod}{Riccardo}{R\bibinitperiod}{}{}{}{}}%
        {{hash=f6346d955920ec5a1960d1642c16cc3d}{Melis}{M\bibinitperiod}{Claudio}{C\bibinitperiod}{}{}{}{}}%
        {{hash=1f1577d1c435291738552646eb1411c1}{Colombo}{C\bibinitperiod}{Luciano}{L\bibinitperiod}{}{}{}{}}%
        {{hash=68031200a434b185de664804eaf80730}{Rurali}{R\bibinitperiod}{Riccardo}{R\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{efb2283ac6e715962672acf6c6630d6e}
      \strng{fullhash}{a45e5655284f70570da0433dd28cf6e0}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{eid}{013107}
      \field{journaltitle}{Applied Physics Letters}
      \field{number}{1}
      \field{title}{Thermal transport in porous Si nanowires from approach-to-equilibrium molecular dynamics calculations}
      \field{volume}{109}
      \field{year}{2016}
    \endentry
    \entry{Yuping2012}{article}{}
      \name{author}{4}{}{%
        {{hash=f325227638798238bccfcac6d9937694}{He}{H\bibinitperiod}{Yuping}{Y\bibinitperiod}{}{}{}{}}%
        {{hash=3c0d859bc38d73ac48e9b8acb09104d7}{Savic}{S\bibinitperiod}{Ivana}{I\bibinitperiod}{}{}{}{}}%
        {{hash=7cf8879ea5293a6c1194f0daec306014}{Donadio}{D\bibinitperiod}{Davide}{D\bibinitperiod}{}{}{}{}}%
        {{hash=a445f4adf3884b1260180426357334a6}{Galli}{G\bibinitperiod}{Giulia}{G\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {The Royal Society of Chemistry}%
      }
      \strng{namehash}{321d8cb0f10ad2bb8e49b5978d1a9df3}
      \strng{fullhash}{f0c05b3bd13db9f6ecc82d4e4652e887}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{47}
      \field{journaltitle}{Phys. Chem. Chem. Phys.}
      \field{title}{Lattice thermal conductivity of semiconducting bulk materials: atomistic simulations}
      \field{volume}{14}
      \field{year}{2012}
      \field{pages}{16209\bibrangedash 16222}
      \range{pages}{14}
    \endentry
    \entry{Hou2016}{article}{}
      \name{author}{4}{}{%
        {{hash=8881091bfb332510cba73fc3a14217e9}{Hou}{H\bibinitperiod}{Chaofeng}{C\bibinitperiod}{}{}{}{}}%
        {{hash=394fcb53d625316e0e80b849469ebbd9}{Xu}{X\bibinitperiod}{Ji}{J\bibinitperiod}{}{}{}{}}%
        {{hash=f7cae3aa58f500a1dd815348f23e8c1e}{Ge}{G\bibinitperiod}{Wei}{W\bibinitperiod}{}{}{}{}}%
        {{hash=2a71c00d3efb730cc9632fac73b73a24}{Li}{L\bibinitperiod}{Jinghai}{J\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{ea7488a288241177c3633a6320339c71}
      \strng{fullhash}{1e2f6c5297176f12ed9a885214ff904f}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Modelling and Simulation in Materials Science and Engineering}
      \field{number}{4}
      \field{title}{Molecular dynamics simulation overcoming the finite size effects of thermal conductivity of bulk silicon and silicon nanowires}
      \field{volume}{24}
      \field{year}{2016}
      \field{pages}{045005}
      \range{pages}{1}
    \endentry
    \entry{Schelling2002}{article}{}
      \name{author}{3}{}{%
        {{hash=61843048aeae8dba6a0a46006636e038}{Schelling}{S\bibinitperiod}{Patrick\bibnamedelima K.}{P\bibinitperiod\bibinitdelim K\bibinitperiod}{}{}{}{}}%
        {{hash=d56395fa0c9d5882660fe99727b4de86}{Phillpot}{P\bibinitperiod}{Simon\bibnamedelima R.}{S\bibinitperiod\bibinitdelim R\bibinitperiod}{}{}{}{}}%
        {{hash=ebf62a6c95a9ef8821da65b778125980}{Keblinski}{K\bibinitperiod}{Pawel}{P\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{ba6bbfedb4ff9c76aa2f99287ba1d667}
      \strng{fullhash}{ba6bbfedb4ff9c76aa2f99287ba1d667}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{14}
      \field{journaltitle}{Phys. Rev. B}
      \field{month}{04}
      \field{title}{Comparison of atomic-level simulation methods for computing thermal conductivity}
      \field{volume}{65}
      \field{year}{2002}
      \field{pages}{144306}
      \range{pages}{1}
    \endentry
    \entry{Zaoui2016}{article}{}
      \name{author}{4}{}{%
        {{hash=1a1113a12a2a0ae336ec741e6555fbba}{Zaoui}{Z\bibinitperiod}{Hayat}{H\bibinitperiod}{}{}{}{}}%
        {{hash=87456d061db087ccfc19dabade86f441}{Palla}{P\bibinitperiod}{Pier\bibnamedelima Luca}{P\bibinitperiod\bibinitdelim L\bibinitperiod}{}{}{}{}}%
        {{hash=fb100d9e4ba1a0c0362d6cb692581d53}{Cleri}{C\bibinitperiod}{Fabrizio}{F\bibinitperiod}{}{}{}{}}%
        {{hash=6d1cb122db175fccc0fcef77aa464a30}{Lampin}{L\bibinitperiod}{Evelyne}{E\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{dc6dd89e6daa9a64855a55a0a8567f45}
      \strng{fullhash}{6aeea7109995927aa286df23e4428377}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{5}
      \field{journaltitle}{Phys. Rev. B}
      \field{month}{08}
      \field{title}{Length dependence of thermal conductivity by approach-to-equilibrium molecular dynamics}
      \field{volume}{94}
      \field{year}{2016}
      \field{pages}{054304}
      \range{pages}{1}
    \endentry
    \entry{Plimton1995}{article}{}
      \name{author}{1}{}{%
        {{hash=489ae657404ae2a22eccc4f507442f4d}{Plimpton}{P\bibinitperiod}{Steve}{S\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{489ae657404ae2a22eccc4f507442f4d}
      \strng{fullhash}{489ae657404ae2a22eccc4f507442f4d}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{0021-9991}
      \field{journaltitle}{Journal of Computational Physics}
      \field{number}{1}
      \field{title}{Fast Parallel Algorithms for Short-Range Molecular Dynamics}
      \field{volume}{117}
      \field{year}{1995}
      \field{pages}{1\bibrangedash 19}
      \range{pages}{19}
    \endentry
    \entry{Shukla2008}{article}{}
      \name{author}{5}{}{%
        {{hash=467f50e8ed6e580f2d817cb6d5f22ff3}{Shukla}{S\bibinitperiod}{P.}{P\bibinitperiod}{}{}{}{}}%
        {{hash=25dbe57fc395454737634b233e57d116}{Watanabe}{W\bibinitperiod}{T.}{T\bibinitperiod}{}{}{}{}}%
        {{hash=1355ac4ffaa6b5156a44356c2cdbf6bb}{Nino}{N\bibinitperiod}{J.C.}{J\bibinitperiod}{}{}{}{}}%
        {{hash=0533053f3176a1d1f00d7735315ad0bf}{Tulenko}{T\bibinitperiod}{J.S.}{J\bibinitperiod}{}{}{}{}}%
        {{hash=1e050447829cab5db555e63bfa72dfe4}{Phillpot}{P\bibinitperiod}{S.R.}{S\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{6d23876a23267e42d9270ffe69499966}
      \strng{fullhash}{8c4278a6d8838fce241f3ca66b45b1f9}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{0022-3115}
      \field{journaltitle}{Journal of Nuclear Materials}
      \field{number}{1–3}
      \field{title}{Thermal transport properties of MgO and Nd2Zr2O7 pyrochlore by molecular dynamics simulation}
      \field{volume}{380}
      \field{year}{2008}
      \field{pages}{1\bibrangedash 7}
      \range{pages}{7}
    \endentry
    \entry{Gygi2008}{article}{}
      \name{author}{1}{}{%
        {{hash=b24c4ceafd5df6270d987ac158711858}{Gygi}{G\bibinitperiod}{F.}{F\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{b24c4ceafd5df6270d987ac158711858}
      \strng{fullhash}{b24c4ceafd5df6270d987ac158711858}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{0018-8646}
      \field{journaltitle}{IBM Journal of Research and Development}
      \field{month}{01}
      \field{number}{1.2}
      \field{title}{Architecture of Qbox: A scalable first-principles molecular dynamics code}
      \field{volume}{52}
      \field{year}{2008}
      \field{pages}{137\bibrangedash 144}
      \range{pages}{8}
    \endentry
    \entry{Kanamori1968}{article}{}
      \name{author}{3}{}{%
        {{hash=fce24e66f39d82ad730be62de3d12ecb}{Kanamori}{K\bibinitperiod}{Hiroo}{H\bibinitperiod}{}{}{}{}}%
        {{hash=e5dffddcf12a49b6044d84663c28f532}{Fujii}{F\bibinitperiod}{Naoyuki}{N\bibinitperiod}{}{}{}{}}%
        {{hash=2c028cbe9b43e9237765a4703494ac96}{Mizutani}{M\bibinitperiod}{Hitoshi}{H\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{241d06aa8ceb5d1a0f5f23eb2f1b7474}
      \strng{fullhash}{241d06aa8ceb5d1a0f5f23eb2f1b7474}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{2156-2202}
      \field{journaltitle}{Journal of Geophysical Research}
      \field{number}{2}
      \field{title}{Thermal diffusivity measurement of rock-forming minerals from 300 to 1100 K}
      \field{volume}{73}
      \field{year}{1968}
      \field{pages}{595\bibrangedash 605}
      \range{pages}{11}
      \keyw{Tectonophysics: Heat flow,General or miscellaneous}
    \endentry
    \entry{Perdew1996}{article}{}
      \name{author}{3}{}{%
        {{hash=f7d11de7da27036e0c12d4055b2fb92d}{Perdew}{P\bibinitperiod}{John\bibnamedelima P.}{J\bibinitperiod\bibinitdelim P\bibinitperiod}{}{}{}{}}%
        {{hash=33a535778ce96cdd2d59799deeea173d}{Burke}{B\bibinitperiod}{Kieron}{K\bibinitperiod}{}{}{}{}}%
        {{hash=ccb694b80578a814211265eb307fdcde}{Ernzerhof}{E\bibinitperiod}{Matthias}{M\bibinitperiod}{}{}{}{}}%
      }
      \list{publisher}{1}{%
        {American Physical Society}%
      }
      \strng{namehash}{1acfabd837046dffa1a0fc3d22c2f827}
      \strng{fullhash}{1acfabd837046dffa1a0fc3d22c2f827}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issue}{18}
      \field{journaltitle}{Phys. Rev. Lett.}
      \field{month}{10}
      \field{title}{Generalized Gradient Approximation Made Simple}
      \field{volume}{77}
      \field{year}{1996}
      \field{pages}{3865\bibrangedash 3868}
      \range{pages}{4}
    \endentry
    \entry{Katsura1997}{article}{}
      \name{author}{1}{}{%
        {{hash=1269819087ba60ad736014454e69a831}{Katsura}{K\bibinitperiod}{Tomoo}{T\bibinitperiod}{}{}{}{}}%
      }
      \strng{namehash}{1269819087ba60ad736014454e69a831}
      \strng{fullhash}{1269819087ba60ad736014454e69a831}
      \field{sortinit}{0}
      \field{sortinithash}{990108227b3316c02842d895999a0165}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{0031-9201}
      \field{journaltitle}{Physics of the Earth and Planetary Interiors}
      \field{number}{1}
      \field{title}{Thermal diffusivity of periclase at high temperatures and high pressures}
      \field{volume}{101}
      \field{year}{1997}
      \field{pages}{73\bibrangedash 77}
      \range{pages}{5}
    \endentry
  \endsortlist
\endrefsection
\endinput


